Restless reachability problems in temporal graphs

We study a family of reachability problems under waiting-time restrictions in temporal and vertex-colored temporal graphs. Given a temporal graph and a set of source vertices, we find the set of vertices that are reachable from a source via a time-respecting path, where the difference in timestamps between consecutive edges is at most a resting time. Given a vertex-colored temporal graph and a multiset query of colors, we find the set of vertices reachable from a source via a time-respecting path such that the vertex colors of the path agree with the multiset query and the difference in timestamps between consecutive edges is at most a resting time. These kind of problems have applications in understanding the spread of a disease in a network, tracing contacts in epidemic outbreaks, finding signaling pathways in the brain network, and recommending tours for tourists, among other. We present an algebraic algorithmic framework based on constrained multi\-linear sieving for solving the restless reachability problems we propose. In particular, parameterized by the length $k$ of a path sought, we show that the proposed problems can be solved in $O(2^k k m \Delta)$ time and $O(n \Delta)$ space, where $n$ is the number of vertices, $m$ the number of edges, and $\Delta$ the maximum resting time of an input temporal graph. In addition, we prove that our algorithms for the restless reachability problems in vertex-colored temporal graphs are optimal under plausible complexity-theoretic assumptions. Finally, with an open-source implementation, we demonstrate that our algorithm scales to large graphs with up to one billion temporal edges, despite the problems being NP-hard. Specifically, we present extensive experiments to evaluate our scalability claims both on synthetic and real-world graphs. Our implementation is efficiently engineered and highly optimized.

==> tikz/tikz-defs.tex <==
\tikzstyle{exedge}  = [draw = yafcolor5!100, thick, text=black!100]
\tikzstyle{exedget} = [draw = yafcolor5!20, thick, text=black!20]
\tikzstyle{exedgedir} = [draw = yafcolor5!20, thick, text=black!20, latex-latexnew, arrowhead=5mm]

\tikzstyle{exnode}  = [thick, draw = black, fill=yafcolor2!05, font = \large,  circle, inner sep = 1pt, text=black, minimum width=14pt]
\tikzstyle{exnodet} = [thick, draw = yafcolor4!20, fill=yafcolor2!02, font = \large,  circle, inner sep = 1pt, text=black!20, minimum width=14pt]
\tikzstyle{exlabel} = [circle, inner sep = 1pt,  font = \large, text = black, auto]
\tikzstyle{exsource}  = [thick, draw = red, fill=yafcolor2!05, font =\large, inner sep = 1pt, text=black, minimum width=14pt, minimum height=14pt]
\tikzstyle{exsquare}  = [thick, draw = yafcolor4!20, fill=yafcolor2!05, font =\large, inner sep = 1pt, text=black, minimum width=14pt, minimum height=14pt]
\tikzstyle{exdiamond}  = [thick, draw = yafcolor4!20, fill=yafcolor2!05, font =\large, inner sep = 1pt, diamond, text=black, minimum width=18pt, minimum height=18pt]

\tikzstyle{label}  = [fill=white, minimum width=0pt, inner sep = 0pt]


\tikzstyle{node1}  = [thick, draw = yafcolor1!100, fill=yafcolor1!05, circle, inner sep = 2.8pt]
\tikzstyle{node2}  = [thick, draw = yafcolor2!100, fill=yafcolor2!05, circle, inner sep = 2.8pt]
\tikzstyle{node3}  = [thick, draw = yafcolor3!100, fill=yafcolor3!05, circle, inner sep = 2.8pt]
\tikzstyle{node4}  = [thick, draw = yafcolor4!100, fill=yafcolor4!05, circle, inner sep = 2.8pt]
\tikzstyle{node5}  = [thick, draw = yafcolor5!100, fill=yafcolor5!05, circle, inner sep = 2.8pt]
\tikzstyle{node7}  = [thick, draw = yafcolor7!100, fill=yafcolor7!05, circle, inner sep = 2.8pt]
\tikzstyle{node8}  = [thick, draw = yafcolor8!100, fill=yafcolor8!05, circle, inner sep = 2.8pt]


\tikzstyle{node}  = [thick, draw = black!100, fill=yafcolor2!05, font = \large,  circle, inner sep = 1pt, text=black, minimum width=14pt]
\tikzstyle{mnode}  = [thick, draw = black!100, fill=yafcolor2!05, font = \large,  circle, inner sep = 1pt, text=black, minimum width=10pt]

